Improvement Graph Convolution Collaborative Filtering with Weighted addition input

Graph Neural Networks have been extensively applied in the field of machine learning to find features of graphs, and recommendation systems are no exception. The ratings of users on considered items can be represented by graphs which are input for many efficient models to find out the characteristics of the users and the items. From these insights, relevant items are recommended to users. However, user's decisions on the items have varying degrees of effects on different users, and this information should be learned so as not to be lost in the process of information mining. In this publication, we propose to build an additional graph showing the recommended weight of an item to a target user to improve the accuracy of GNN models. Although the users' friendships were not recorded, their correlation was still evident through the commonalities in consumption behavior. We build a model WiGCN (Weighted input GCN) to describe and experiment on well-known datasets. Conclusions will be stated after comparing our results with state-of-the-art such as GCMC, NGCF and LightGCN. The source code is also included at https://github.com/trantin84/WiGCN.

==> NotesVietnamese.tex <==
Các hệ thống khuyến nghị là một lĩnh vực nghiên cứu quan trọng của Hệ thống thông tin. Chúng được sử dụng rộng rãi trong thương mại điện tử, quảng cáo và truyền thông xã hội ... nhằm đưa ra những gợi ý cho người dùng mục tiêu, và vì thế, nâng cao trải nghiệm người dùng. Dựa trên tương tác, chẳng hạn như mua hàng hay đánh giá, trước đây của nhiều người dùng trên các mặt hàng mà hệ thống sẽ tìm kiếm những đặc trưng và chỉ ra những người dùng tương tự và mặt hàng tương tự để đưa ra tập hợp các sản phẩm và gợi ý đến khách hàng mục tiêu. Lọc cộng tác (CF) là phương pháp đánh giá mức độ giống nhau giữa những người dùng dựa trên chuỗi hành vi trong quá khứ đã được áp dụng trong 1,2,3 ; trong phương pháp này, đặc trưng của người dùng và mặt hàng được biểu diễn vecto . Khoảng cách các vector trong không gian miêu tả thể hiện mức độ tương đồng của người dùng hoặc mặt hàng. Độ đo này có thể là cos, fd, dfds (distance VIET THEM)

Ma trận quan hệ người dùng và mặt hàng thường là ma trận thưa, bởi vì số mặt hàng một người dùng đã mua hay đã quan tâm chỉ chiếm tỉ lệ rất nhỏ so với tất cả các mặt hàng. Việc thu giảm số chiều ma trận giúp cho tạo ra các ma trận nhúng có kích thước nhỏ hơn rất nhiều nhưng không làm mất đặc trưng của người dùng và mặt hàng [10]. Hơn nữa, các thư viện Numpy, Scipy và Tensorflow [tham khao] có thể xử lý hiệu quả các ma trận thưa kích thước rất lớn mà không chiếm nhiều bộ nhớ máy tính khi thực thi.

Bên ngoài khuyến nghị truyền thống, khuyến nghị xã hội là các hệ thống xem xét thêm yếu tố thân thiết giữa các người sử dụng. Các người dùng cũng có thể là bạn bè của nhau trong cuộc sống thực hay trên mạng xã hội, lời khuyên của một người bạn luôn được tiếp đón với mức độ khác nhau. Các phương pháp được nêu ở [SO REG/ SO REC] đã khai thác cơ sở dữ liệu quan hệ bạn bè để làm giàu thông tin khuyến nghị.

Mặt khác, quan hệ người dùng và các mặt hàng cũng có thể biểu diễn một cách tự nhiên bởi đồ thị, và có thể được khai thác bởi GNN theo công bố [gnn] hoặc [gcn]. Quá trình ghi nhận các tín hiệu cộng tác có thể qua hai giai đoạn là decomposer và combiner như đề xuất tại [mccf], trong đó decomposer sẽ ghi nhận các tín hiệu từ đồ thị và sau đó, combiner sẽ liên kết chúng thành một unified embedding. High-order connectivity được tìm thấy trong mô hình [ngcf] khi mà propagating embedding được sử dụng khi khai thác đồ thị quan hệ người dùng và mặt hàng. Gần đây, mô hình LightGCN [lighGCN] đã loại bỏ các trọng số khi thu nhận tín hiệu từ đồ thị vào các vector nhúng nhưng vẫn giữ được độ chính xác của giải thuật.


---------------------- CF --------------
Những giải pháp đầu tiên của các hệ thống khuyến nghị đã khai thác các đặc trưng của mọi đối tượng cũng như sở thích của các người dùng để tìm kiếm các mặt hàng phù hợp và đưa ra khuyến nghị \cite{Jalili18}. Ví dụ một bộ phim có thể mang thuộc tính thể loại hành động, hài kịch, lãng mạn, ... một món đồ chơi có thể mang thuộc tính màu sắc, hình dạng, độ tuổi phù hợp, ... Về phía người dùng, những thông tin như độ tuổi, giới tính, nơi cư trú hay học vấn cũng được sử dụng để làm giàu thông tin cho đầu vào. [32/33 of Jalili] Tuy nhiên, với số lượng mặt hàng rất lớn và được bổ sung thường xuyên, việc gán nhãn (gán thuộc tính) cho các mặt hàng gặp nhiều khó khăn, các hệ thống cần những phương phá lọc cộng tác (34) để tìm kiếm sự tương đồng giữa những người sử dụng hoặc là các mặt hàng mà không cần các thông tin thuộc tính.

Lọc cộng tác có thể dựa trên memory-based(35)  hoặc là trên mô hình (34). Với memory- based, lịch sử đánh giá của mọi người dùng lên các mặt hàng sẽ được ghi nhớ lại trong một ma trận đánh giá. Có nhiều cách định nghĩa thang đánh giá, có thể là giá trị nguyên từ 1 đến 5, hoặc là implict chỉ là có hoặc không. Trong không gian tạo thành từ tập người dùng, tập món hàng và các giá trị đánh giá, mỗi người dùng được biển diễn bằng một vector đặc trưng eu, cũng như mỗi món hàng được biễn diễn bằng vector đặc trưng ei. Các giải thuật sẽ dựa trên khoảng cách giữa mỗi cặp người dùng (hay món hàng đối với item based) để tìm ra những lân cận và hình thành nên kết quả khuyến nghị. Khoảng cách có thể là độ tương tự cosine, Pearson hay Euclidean và MSD. Sự khó khăn của các phương pháp này là bộ nhớ khó chứa nổi ma trận dữ liệu nhập và và ma trận này có tính chất thưa thớt do một người dùng thường chỉ đánh giá một vài mặt hàng nào đó.

Còn đối với lọc cộng tác dựa trên mô hình, các giải thuật sẽ tìm kiếm khuôn mẫu của dữ liệu học để tạo ra một mô hình cho dự đoán trong tương lai. (36,89,90). Phương pháp phân tích ma trận có thể áp dụng để thu giảm số chiều của ma trận dữ kiện đánh giá người dùng lên các mặt hàng. Ma trận đánh giá có thể được phân tách thành ma trận đặc trưng người dùng và ma trận đặc trưng mặt hàng với kích thước nhỏ hơn; nhưng vẫn đảm bảo độ chính xác của khoảng cách giữa các người dùng cũng như giữa các mặt hàng, thậm chí kết quả dự đoán khuyến nghị còn tốt hơn (theo 113), khả năng mở rộng và quá trình học dữ liệu dễ dàng hơn.

SVD / NMF

Độ đo lượng giá sẽ được chọn lựa phù hợp cho từng giải thuật(4/132). Một phương pháp thường được sử dụng là trích xuất một phần của tập dữ liệu để tạo thành tập kiểm tra, phần còn lại là tập huấn luyện.   Giải thuật được áp dụng trên tập huấn luyện để đưa ra các dự đoán đánh giá trên tập kiểm tra. Sự sai khác giữa kết quả học và giá trị dữ liệu thực tế nói lên độ chính xác của giải thuật. Sự sai khác này có thể tính bằng MAE hay là RMSE. Bên cạnh độ chính xác, độ bao phủ, tính mở rộng, thời gian học, bộ nhớ tiêu thụ hay khả năng lý giải cũng là những tiêu chí quan trong trong lượng giá hệ thống khuyến nghị.

// công thức MAE và RMSE

Đối với các dữ liệu implict, tương tác giữa người sử dụng và các mặt hàng được ghi nhận nhị phân, thay vì đánh giá là một giá trị cụ thể. Khi đó, các giải thuật sẽ sử dụng độ đo chính xác cho việc phân lớp. Độ đo thường được dùng là Precision và Recall (143,54,75,76,114). 

// công thức P và R

F1 score được sử dụng để cân đối giữa độ chính xác và recall vì hai đại lượng này thường là đối nghịch. (75,76)

Ngoài ra độ đo NGCF = ...

%------viet ve GNN

Mạng neuron đã có những thành công mạnh mẽ trong việc thiết lập các lớp ẩn để trích lọc dữ liệu đầu vào và định ra những đặc trưng của tập dữ liệu ở đầu ra (trích dẫn). Đồ thị là cấu trúc dữ liệu biểu diễn mối quan hệ giữa các thực thể, con người, dữ kiện, thuộc tính bằng cách sử dụng tập đỉnh V để biểu diễn đối tượng và tập cạnh E để biểu diễn mối quan hệ. Một cạnh của đồ thị có thể vô hướng chỉ thể hiện quan hệ, hoặc nêu rõ trọng số của mối quan hệ hoặc là cạnh có hướng. Những nghiên cứu (gnn) đã áp dụng mạng neuron với dữ liệu đầu vào là đồ thị và thu nhận được những kết quả tích cực khi đặc trưng của các đỉnh được lan truyền và aggregated vào lẫn nhau trong quá trình học. (139,161) \cite{9046288}. Thừa kế từ các giải thuật Neural Network, GNN cũng sử dụng nhiều lớp lan truyền và áp dụng các giải pháp aggration và cập nhật khác nhau. Các tính chất của đỉnh lân cận được cập nhật và đỉnh mục tiêu bởi việc pooling hoặc những cơ chế chú ý \cite{GAT}. 

GCN là một phương pháp thu thập các thông tin lặp lại nhiều lần \cite{10.1145/3219819.3219890}. Chẳng hạn như khi có một món hàng cùng được quan tâm bởi nhiều người bạn của người dùng mục tiêu, thì nó nên được khuyến nghị với mức độ cao hơn các mặt hàng khác. GraphSAGE \cite{DBLP:journals/corr/HamiltonYL17} đã inductive nhúng cho mỗi đỉnh của đồ thị và học được cấu trúc topo của đồ thị cũng như sự tác động của đỉnh lên các đỉnh lân cận. This methode not only focus on feature-rich graphs but also make use of structural features of all vertices.

Multi Component Graph Convolutional \cite{MCGC} đã xem đồ thị đầu vào gồm hai thành phần bằng việc phân tách các đỉnh đại diện cho người dùng làm một nhóm và các đỉnh đại diện cho mặt hàng là nhóm còn lại. Đặc trưng của các người sử dụng được tính toán để nhúng vào nhau và đặc trưng của các mặt hàng cũng vậy. Quá trình học được chia làm 2 giai đoạn chính: decomposer và conbiner. Trong đó, thành phần decomposer sẽ thu nhận một số luọng M latent từ ma trận quan hệ người dùng-mặt hàng thông qua M ma trận chuyển đổi và tổng hợp vào các đỉnh người dùng (hay là mặt hàngu. Thành phần combiner sẽ kết hợp các vector đặc trưng của các mặt hàng lên một người dùng cụ thể và của các người dùng lên một mặt hàng cụ thể. Cuối cùng hệ thống có được đánh giá dự đoán ở đầu ra.

Với giả thuyết rằng sự ảnh hưởng của các người dùng là khác nhau tuỳ vào khoảng cách giữa các đỉnh trong đồ thị, Neural Graph Collaborative Filtering \cite{NGCF} tạo ra các lớp lan truyền theo từng hop trong đồ thị đầu vào. Lớp lan truyền thứ k-th được gọi là k-order propagation, thu nhận các thông điệp từ các mặt hàng đến một người dùng cũng những những tín hiệu chú ý từ các lân cận của người dùng đó. Số lớp lan truyền k có thể xem là thông số đầu vào và giá trị k=3 được xem là tối ưu nhất.  Hàm mất mát được xây dựng từ sự sai khác của bộ giá trị đánh giá dự đoán và thực tế của tập kiểm tra. Quá trình học nhằm cực tiểu hàm mất mát được diễn ra sau một số lần lặp tuỳ thuộc vào tốc độ học, kích thước các ma trận nhúng cũng như kích thước dữ liệu học. Trong một phiên bản tiếp theo của NGCF, LightGCN \cite{he2020lightgcn} đã loại bỏ các ma trận trọng số chuyển đổi đặc trưng trong quá trình lan truyền , và hàm activation non-linear để cắt bỏ những negative effect lên các đối tượng trong quá trình lan truyền. 




==> note_err.tex <==
>>> 1. Language problems:

1.1 Tensorflow => TensorFlow

1.2 "important criterias" => "important criteria"

1.3 optimazation => optimization

1.4 mesages => messages

1.5 trainning => training

1.6 expriment => experiment

1.7 "We config our model" => "We configure our model "

1.8 AdamOptimization => "Adam algorithm"

1.9 decomposion => decomposition

1.10 comparasion => comparison

1.11 "We gives statics of these dataset af Table 1."
grammar

1.12 "In most of cases, 3-layers gives the best score."
grammar

1.13 "in almost cases."
in almost all cases or in almost none cases?


>>> 2. Presentation problems:

2.1 format of references is not consistent. Please compare e.g. [19, 26] and [22, 28]

2.2 Table 2: title is too general. It is not clear if presented results were obtained for training or test data.

2.3 Fig 3: title is too general. It is not clear which results are related to MF.


>>> 3. Other problems:

3.1 Authors write: "We hope that"
In scientific document Authors should not write about their hopes or other feelings - just about facts and/or hypotheses.

3.2 Authors write: "Trust weight graphs between users , which were prepared and send into the
proposed computational model, based on the interactions of many users on the same item."

The meaning of this sentence is unclear.

3.3 Results (Table 2) are given without confidence intervals. This can make comparisons of values biased.

3.4 Why F1 measure is defined in (2) while it is not used in the rest of the document?

3.5 Authors write: "Rectified Linear Unit activation function"

It is a fact that in many publications the term ReLU (Rectified Linear Unit) is used as the name of type of activation function. But it can be easily found that such usage of "ReLU" term is improper. See the list of publications given below - including the publication of Hinton and Nair who proposed usage of Rectified Linear Units in deep learning. It clearly shows that the term "unit" refers to "neuron" and the Rectifier Linear function (in short: Rectifier or ReL) is used as the activation function within neurons. In the result ReLU is a unit (neuron) which uses Rectifier Linear activation function. Even if some existing publications mismatch ReLU with Rectifier Linear function Authors should not include such an error within their publication.

1.) Vinod Nair and Geoffrey Hinton (2010). Rectified Linear Units Improve Restricted Boltzmann Machines. ICML:
Authors clearly express that "unit" means "a neuron", e.g. they write: "a hidden unit".
See: https://www.cs.toronto.edu/~hinton/absps/reluICML.pdf

2.) Xavier Glorot, Antoine Bordes and Yoshua Bengio, "Deep Sparse Rectifier Neural Networks", AISTATS 2011, pp. 315-323:

"(..) machine learning neural network models can be bridged by using the following linear by part activation : max(0, x), called the rectifier activation function."

3.) Yangwei Wu Haohua Zhao Liqing Zhang, "Image Denoising with Rectified Linear Units",
International Conference on Neural Information Processing, ICONIP 2014, pp 142-149:

"In this paper, we adopt the rectified linear (ReL) function instead of the sigmoid function as the activation function of hidden layers to further enhance the ability of neural network on solving image denoising problem."

See: https://link.springer.com/chapter/10.1007/978-3-319-12643-2_18

4.) OReilly library:

"A neuron uses a rectifier is known as a rectified linear unit (ReLU)."

See: https://www.oreilly.com/library/view/machine-learning-with/9781787121515/0d797ec1-539d-48b0-a738-109c76e8ff70.xhtml

5.) Wikipedia:

"A unit employing the rectifier is also called a rectified linear unit (ReLU)."

See: https://en.wikipedia.org/wiki/Rectifier_(neural_networks)

6.) machinelearningmastery.com:

"A node or unit that implements this (Rectified Linear) activation function is referred to as a rectified linear activation unit"

See: https://machinelearningmastery.com/rectified-linear-activation-function-for-deep-learning-neural-networks


>>>> Summary:

Language and presentation need many fixes and improvements. Presented idea is interesting, but statistical analysis of results is very shallow. This can make conclusions biased and not fully backed up by presented data.

Recommendation: weak reject 

===EOT===
